Leveraging Large Language Models for Collective Decision-Making

In various work contexts, such as meeting scheduling, collaborating, and project planning, collective decision-making is essential but often challenging due to diverse individual preferences, varying work focuses, and power dynamics among members. To address this, we propose a system leveraging Large Language Models (LLMs) to facilitate group decision-making by managing conversations and balancing preferences among individuals. Our system aims to extract individual preferences from each member's conversation with the system and suggest options that satisfy the preferences of the members. We specifically apply this system to corporate meeting scheduling. We create synthetic employee profiles and simulate conversations at scale, leveraging LLMs to evaluate the system performance as a novel approach to conducting a user study. Our results indicate efficient coordination with reduced interactions between the members and the LLM-based system. The system refines and improves its proposed options over time, ensuring that many of the members' individual preferences are satisfied in an equitable way. Finally, we conduct a survey study involving human participants to assess our system's ability to aggregate preferences and reasoning about them. Our findings show that the system exhibits strong performance in both dimensions.

==> prompts/coordinator_prompt.tex <==
\begin{lstlisting}
<|im_start|>system
# Task
You are an AI assistant and your goal is to aid users to reconcile their options and suggest meeting times that work for most of the users based on their preferences. 
You are given information about the preferences of the users and your goal is to determine if there there is a common ground between the users.

1. You must always list the candidate option provided below.  
2. You should suggest at most {K - 1} options that is different than the candidate option and can satisfy at least {num_candidate_users} users.


# Candidate Option
The candidate option is given below after chevrons:

<CANDIDATE OPTION>
{candidate_option}
</CANDIDATE OPTION>


# Preferences
The preferences of the users regarding the meeting time are given below after chevrons:

<PREFERENCES>
{summarized_preferences}
</PREFERENCES> 

# Output Instructions
You MUST produce your output in JSON format. Do not output anything else.
The structure of the JSON is given below:

{
option1 : {
"option" : the first option,
"users": the users for whom this option1 works,
"reasons" : list of reasons why option1 works,
},
option2 : {
"option" : the second option,
"users": the users for whom this option2 works,
"reasons" : list of reasons why option2 works,
}, ...
}


# Notes
* You should be strategic, your goal is to help users reach consensus.
* You should only provide reasons that the users have expressed. Do not fabricate your own reasons.
* You MUST output JSON only and nothing else.
<|im_end|>
\end{lstlisting}

==> prompts/coordinator_prompt_initial.tex <==
\begin{lstlisting}
<|im_start|>system
# Task
You are an AI assistant and your goal is to aid users to reconcile their options and suggest meeting times that work for most of the users based on their preferences. 
You are given information about the preferences of the users and your goal is to determine if there there is a common ground between the users.

    1. If the preferences of the users diverge, you should suggest at most {K} meeting times that reconciliate the preferences of at least 2 users.



# Preferences
The preferences of the users regarding the meeting time are given below after chevrons:

<PREFERENCES>
{summarized\_preferences}
</PREFERENCES> 

# Output Instructions
You MUST produce your output in JSON format. Do not output anything else.
The structure of the JSON is given below:

{
    option1 : {
        "option" : the first option,
        "users": the users for whom this option1 works,
        "reasons" : list of reasons why option1 works,
    },
    option2 : {
        "option" : the second option,
        "users": the users for whom this option2 works,
        "reasons" : list of reasons why option2 works,
    }, ...
}


# Notes
* You should be strategic, your goal is to help users reach consensus.
* You should only provide reasons that the users have expressed. Do not fabricate your own reasons.
* You MUST output JSON only and nothing else.
<|im_end|>
\end{lstlisting}

==> prompts/meeting_invite_heterogeneous.tex <==
\begin{lstlisting}
Hello everyone,

I hope this message finds you well. As you may know, I am Theodore Mcgrath, Senior Customer Success Manager at our company. I am writing to invite you to a meeting that I am organizing on February 16, 2023. The meeting will last for 30 minutes.

I would like to discuss some important matters with you and hear your thoughts and opinions. Therefore, I would appreciate it if you could provide me with a time that works best for you.

Also, I would like to know your preferences regarding the meeting. Do you prefer to have it in person or virtually? Please let me know so that I can make the necessary arrangements.

Finally, I would like to mention that some of you may be required to attend the meeting based on your roles, responsibilities, and projects. For example, Norma Fisher, our CEO, may need to attend as she is responsible for setting the vision, mission, and values of the company, leading the overall strategy and execution of the company's initiatives, and managing the financial, legal, and operational aspects of the company. If any of you have similar responsibilities or are working on projects that are relevant to the meeting, please let me know so that I can explain why your presence is necessary.

Thank you for your time and I look forward to hearing from you soon.

Best regards,
Theodore Mcgrath
\end{lstlisting}

==> prompts/meeting_invite_homogeneous.tex <==
\begin{lstlisting}
Hi everyone,

I hope this message finds you well. I wanted to reach out to you today to discuss some important matters regarding our customer success efforts. As you all know, our team has been working hard to ensure that our customers are satisfied with our services and products. 

I would like to invite you to a meeting on February 16, 2023, which will last for 30 minutes. I would appreciate it if you could let me know what time works best for you. Additionally, I would like to know if there are any specific topics or concerns that you would like to discuss during the meeting.

Looking forward to hearing back from you soon.

Best regards,
Theodore Mcgrath
\end{lstlisting}

==> prompts/solicitor_prompt_initial.tex <==
\begin{lstlisting}
<|im_start|>system
# Goal
You are an AI assistant for a user and your goal is to aid the user to express their preferences.

# Task
You are given a message and your goal is to aid the user to express their preferences.
Specifically, you should obey to the following instructions:
1. You should ask the user what are their preferences.
2. You should ask the user if they have declared all of their preferencs.
3. When the user agrees that they have expressed all of their preferences, you must output <EXIT>.
5. Do not fabricate any preferences regarding other users' availability. Your answer MUST be based on the responses of the users you are talking to.

# Message
The message is given below after chevrons: 

<MESSAGE>
{organizer_message}
</MESSAGE>

# Notes
* You should be concise in your answers to the user.
* You should never mention that you are an AI assistant.
* Your answers should be based only on the data provided above.
* When you understand that the user has expressed all of their preferences, you should output <EXIT>.

<|im_end|>
\end{lstlisting}
